Corps: A Core Calculus of Hierarchical Choreographic Programming

Functional choreographic programming suggests a new propositions-as-types paradigm might be possible. In this new paradigm, communication is not modeled linearly; instead, ownership of a piece of data is modeled as a modality, and communication changes that modality. However, we must find an appropriate modal logic for the other side of the propositions-as-types correspondence. This paper argues for doxastic logics, or logics of belief. In particular, authorization logics -- doxastic logics with explicit communication -- appear to represent hierarchical choreographic programming. This paper introduces hierarchical choreographic programming and presents Corps, a language for hierarchical choreographic programming with a propositions-as-types interpretation in authorization logic.

==> Makefile <==
BIB := main.bib

PAPER_FILES := $(find . -name "*.tex")

export TEXINPUTS = .::$TEXMF/tex/

.PHONY: clean cleanall

corps.pdf: main.tex $(PAPER_FILES) $(BIB)
	latexmk -pdf -bibtex -synctex=1 -jobname=corps $<


ALLCLEANABLES := $(shell find . \( -name '*.aux'\
                             -o -name '\#*\#'\
			     -o -name '*.log'\
			     -o -name '*.bbl'\
                             -o -name '*.out'\
                             -o -name '*~'\
                             -o -name '*.pdf'\
                             -o -name '*.dvi'\
                             -o -name '*.synctex.gz'\
                             -o -name '*.blg'\
                             -o -name 'paper-outline.tex'\
                             -o -name '*.toc'\
                             -o -name '*.lot'\
			     -o -name '*.fls'\
			     -o -name '*.rip'\
			     -o -name '*.fdb_latexmk'\
			     -o -name '*.xcp'\
			     -o -name '*.xoj'\
                             -o -name '*.lof' \) -type f)

CLEANABLES := $(shell find . \( -name '*.aux'\
			     -o -name '\#*\#'\
			     -o -name '*.log'\
			     -o -name '*.bbl'\
                             -o -name '*.out'\
                             -o -name '*~'\
                             -o -name '*.synctex.gz'\
                             -o -name '*.blg'\
                             -o -name 'paper-outline.tex'\
                             -o -name '*.toc'\
                             -o -name '*.lot'\
			     -o -name '*.fls'\
			     -o -name '*.rip'\
			     -o -name '*.fdb_latexmk'\
			     -o -name '*.xcp'\
                             -o -name '*.lof' \) -type f)

clean: 
	@for f in $(CLEANABLES); do \
		echo "REMOVING $$f";\
		rm $$f;\
	done

cleanall: 
	@for f in $(ALLCLEANABLES); do \
		echo "REMOVING $$f";\
		rm $$f;\
	done


==> appendices.tex <==
% include appendices, similar to sections.tex


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "conference"
%%% End:

